Smoothed complexity of local Max-Cut and binary Max-CSP

We show that the smoothed complexity of the FLIP algorithm for local Max-Cut is at most $\smash{\phi n^{O(\sqrt{\log n})}}$, where $n$ is the number of nodes in the graph and $\phi$ is a parameter that measures the magnitude of perturbations applied on its edge weights. This improves the previously best upper bound of $\phi n^{O(\log n)}$ by Etscheid and R\"{o}glin. Our result is based on an analysis of long sequences of flips, which shows~that~it is very unlikely for every flip in a long sequence to incur a positive but small improvement in the cut weight. We also extend the same upper bound on the smoothed complexity of FLIP to all binary Maximum Constraint Satisfaction Problems.

==> introduction_old.tex <==
% !TEX root =  main.tex

\section{Introduction}

Local search is one of the most prominent algorithm design paradigms for combinatorial optimization problems.
Such an algorithm begins with an initial solution and then follows a path by iteratively moving to~a better neighboring solution  
  until a local optimum is reached. 
Many algorithms currently deployed in practice, including many for machine learning tasks such as ??,
  are based on local search, and all the empirical evidence suggests that they typically perform very well in practice,
  rarely running into long paths before reaching a local optimum.
  
%To encapsulate many local search problems, Johnson et.al. \cite{johnson1988easy} introduced the complexity class PLS (polynomial local search) and initially showed PLS-completeness for the circuit-flip problem. Sch$\ddot{\text{a}}$ffer and Yannakakis \cite{schaffer1991simple} extended the research on PLS and sho
However, despite their wide success in practice, the performance of many local search algorithms lacks
  rigorous justifications. % and in particular, the classical worst-case analysis framework typically does not work
A recurring phenomenon is that an algorithms performs very well in practice but
  at the same time is shown to have exponential running time in the worst case due to 
  delicate instances that one never expects to encounter in practice. 
A concrete (and probably one of the simplest) example for this phenomenon is the \emph{FLIP} algorithm for the \emph{local max-cut} problem.
%A recurring phenomenon is that man algorithms runs efficiently in practice but is shown to have 
 % exponential running time in the worst case.
%To bridge this gap,
%  the smoothed analysis framework was introduced by 
 % Spielman and Teng \cite{} to 
 %  provide rigorous
 % justifications for the good practical performance of the simplex
%  algorithm, even though it is known to be exponential-time in the worst case \cite{KleeMinty} (a recurring theme
 % for many other local search algorithms such as ? and ?). 
%Essentially a local search algorithm, 
%  the success of smoothed analysis 
%Informally, the smoothed complexity of an algorithm is measured by 
%  its worst-case expected running time on any instance after a slight random perturbation.
%Since then,
%  the framework has been applied to many 
%They proved that the smoothed complexity of the simplex algorithm with
%the shadow-vertex pivoting rule is polynomial.
%The smoothed analysis framework was introduced by Spielman and Teng in \cite{} to explain 
 % why some algorithms, most notably 
%In their celebrated result \cite{},   
%  the simplex algorithm for linear programming, though 
 % known to take exponential time in the worst case \cite{KleeMinty}, 
 % were nevertheless very fast in practice. 
 
Given an undirected graph $G=(V,E)$ with edge weights $(X_e\in [-1,1]: e\in E)$,
  the local max-cut problem is to find a cut of $V$ into two sets $V_1$ and $V_2$
  such that the weight of the cut cannot be improved by moving one of the nodes to the other side.
To find a local max-cut, the FLIP algorithm starts with an initial cut and keeps moving nodes, one by one,
  until no local improvement can be made. (Note that the FLIP algorithm is really a family of algorithms since one 
  can apply different rules to pick the node to be moved, when more than one nodes can be moved to improve the cut.
  This is similar to the simplex algorithm with a variety of pivoting rules.)
The local max-cut problem is known to be PLS-complete \cite{}, a complexity class introduced by \cite{} to 
  characterize all the local search problems;
a consequence of the completeness result is that FLIP takes exponential time to solve local max-cut in the worst case.
The local max-cut problem can be viewed equivalently as the problem of finding a pure Nash equilibrium in a \emph{party affiliation game} \cite{};
  it also appears in the context of Hopfield networks \cite{}.
Generalizing local max-cut, introduce local binary CSP.
  
In this paper we study the \emph{smoothed complexity} of the FLIP algorithm for local max-cut
  and binary max-CSP.
The smoothed analysis framework was introduced by 
  Spielman and Teng \cite{} to 
  provide rigorous
  justifications for the good practical performance of the simplex
  algorithm, even though it is known to be exponential-time in the worst case \cite{KleeMinty}.
Since then it has been applied in a range of areas; see \cite{}.
Specialized to the local max-cut problem, the input becomes an undirected graph $G=(V,E)$ with
  a vector $\calX=(\calX_e: e\in E)$ of probability distributions.
Each $\calX_e$ is a distribution supported on $[-1,1]$ and its density function is bounded from above
  by a parameter $\phi>0$ (which measures the magnitude of perturbation applied on edge weights).
The question is then to give a bound $t(n,\phi)$ such that for any $G$ and $\calX$,
  the FLIP algorithm terminates within $t(n,\phi)$ steps with high probability (say $1-o_n(1)$)
  over the draw of edge weights $X\sim \calX$ (where each edge weight is drawn independently).
  
The best result for $t(n,\phi)$ before our work is the quasipolynomial upper bound $\phi\cdot n^{O(\log n)}$ 
  by Etscheid and \Roglin \cite{}, based on a rank-based approach which we review in Section \ref{sec:maintheorem}.
Before their work, polynomial upper bounds were obtained by Elsasser and Tscheuschner 
  and by Etscheid and \Roglin for special cases either when $G$ has $O(\log n)$ degree or 
  when $G$ is a complete graph with edge weights given by Euclidean distances.
After the work of \cite{}, Peres \cite{} obtained a polynomial bound for $t(n,\phi)$ when $G$ is a complete graph.
Their polynomial bound was later improved by \cite{}, again for complete graphs.
Both results of \cite{} are based on the rank-based approach at a high level, with new techniques
  that are better suited for complete graphs. 
%For an undirected graph $G = (V, E)$ with weighted edges 
%$w : E \to [-1,1]$ a cut is a partition of $V$ into two sets
%$V_1, V_2$. The weight of the cut is the sum of the weights of the edges connecting nodes between $V_1$ and $V_2$. The max-cut problem asks for a cut of maximum weight. Computing a maximum cut is one of the most famous problems in computer science and is known to be NP-complete even on graphs with maximum degree three. 
%Known to be PLS-complete, but FLIP finishes fast typically.

%A frequently used approach of dealing with hard combinatorial optimization problems is local search. wed PLS-completeness for many popular local search problems including the local max-cut with FLIP-neighborhood.



%More formally, the local max-cut problem asks to find a partition of the vertices 
%$\sigma : V\rightarrow \{-1, 1\}$ whose total cut weight 
%\begin{equation}
  %  \label{equation:local-max-objective}
   % \obj(\sigma)=\frac{1}{2}\displaystyle\sum_{e=(u,v)\in E}w(e)(1-\psi(u)\psi(v))
%\end{equation}
%is locally maximal, in the sense that one cannot increase the cut weight by changing the value of $\sigma$ at a single vertex. On the other hand, the FLIP algorithm iteratively performs improving moves until reaching a configuration with no improving move. An implementation of FLIP specifies how to choose the initial configuration and how to choose among the improving moves available at each step. (Etscheid and \\Roglin
%2014) \cite{etscheid2015smoothed} show that for any graph with smoothed weights, with high probability, any implementation of FLIP will terminate in at most
%$n^{C \log(n)}$ steps, for some universal constant C > 0. Additionally Angel et.al.
%\cite{angel2017local} show that FLIP terminates in a polynomial number of steps for the complete graph. Inspired by the latter work we are able to improve
%Etscheild and \\Roglin's result for an arbitrary graph in $n^{O(\sqrt{\log n})}$.

%We represent a cut by a configuration $\psi$ in 
%$\{\pm1\}^V$ that represents the part of each vertex. A
%move of a vertex from a given configuration can be described using a vector 
%$\gamma \in \{0, \pm1\}^E$ such that the increase in the cut value for that move is given by $\left \langle \gamma,X \right \rangle $, where $X$ is the random vector of weights $[-1,1]^E$. Instead of fixing each edge weight deterministically he can only specify for each edge $e \in E$ a probability density function $f_e : [-1, 1] \to [0, \phi]$ according to which the weight $w(e)$ is chosen independently of the other edge weights. 
%The parameter $\phi \ge 1/2$ determines how powerful the adversary is. 
%He can, for example, choose for each edge weight an interval of length $1/\phi$ from which
%it is chosen uniformly at random. This shows that in the limit for $\phi$ the adversary
%i%s as powerful as in a classical worst-case analysis, whereas the case $\phi = 1/2$ constitutes an average-case analysis with uniformly chosen edge weights. Note that the restriction to the interval $[-1, 1]$ is merely a scaling issue and no loss of generality.



%For a starting configuration
%$\psi_0 \in \{\pm1\}^V$, we define a matrix $P_{L,\psi_0}$
%that conveniently nullifies the effect of non-moving vertices
%of $L$: for each pair of closest moves of a vertex $v$ in $L$, we have a column in $P_{L,\psi_0}$ which is the sum of the two vectors $\gamma_1,\gamma_2$ corresponding to those two moves of $v$. The main advantage of this matrix $P_{L,\psi_0}$
%is that it depends only on the starting configuration of the vertices which move in $L$
%and is independent of the starting configuration of the vertices that do not move in $L$ (Proposition 3.6). This feature is crucially helpful while taking a union bound later. Our matrix $P_{L,\psi_0}$ is also implicitly used by Etscheid and \\Roglin.
%For the rest of the text, $\rank{P_{L,\psi_0}}=\rank{\psi_0,L}$

%State the main theorem in the introduction:
\subsection{Our results}

\begin{theorem}[Main]\label{maintheorem}
Let $G=(V,E)$ be an undirected graph over $n$ vertices and 
  $\calX=(\calX_e:e\in E)$ be a sequence of probability distributions 
  such that every $\calX_e$ is supported on $[-1,1]$ and has density bounded from above by
  a parameter $\phi>0$.
%the edge weights are independent random variables bounded by $[-1,1]$ and has density at most $\phi$, 
Then with probability $1-o_n(1)$ over the draw of $X\sim \calX$,
  any implementation of FLIP running on $G$ and~$X$ takes at most $\phi\cdot n^{O(\sqrt{\log n})}$  steps to terminate.
\end{theorem}

\subsection{The $\log n$-barrier to the rank-based approach}

\subsection{Our techniques}

delicate, balance properties of arcs.

==> octopus.tex <==
\section{Octopus Graph}
Here is a draft which summarize the construction of an interesting case for
the smooth complexity of local maxcut. Firstly, let's define the octopus graph.
\begin{center}
\begin{tikzpicture}
%% vertices
\draw[fill=red] (-2,0) circle (3pt);
\draw[fill=red] (-1,0) circle (3pt);
\draw[fill=red] (1,0) circle (3pt);
\draw[fill=red] (2,0) circle (3pt);
\draw[fill=green] (0,1) circle (3pt);
\draw[fill=red] (-2,3) circle (3pt);
\draw[fill=green] (-1,3) circle (3pt);
\draw[fill=red] (0,3) circle (3pt);
\draw[fill=green] (2,3) circle (3pt);
\draw[fill=red] (4,3) circle (3pt);
\draw[fill=red] (-2,4) circle (3pt);
\draw[fill=green] (-1,4) circle (3pt);
\draw[fill=red] (0,4) circle (3pt);
\draw[fill=green] (2,4) circle (3pt);
\draw[fill=red] (4,4) circle (3pt);

%% vertex labels

\node at (-2.3,-0.3)  {$ v_1 $};
\node at (-1.3,-0.3)  {$ v_2 $};
\node at (0,-0.3)  {$ \cdots \cdots $};
\node at (1.3,-0.3)  {$ v_{n^{0.2}-1} $};
\node at (2.3,-0.3)  {$ v_{n^{0.2}} $};
\node at (0.5,1.3)  {$ u $};
\node at (-2.3,3.3)  {$ w_1 $};
\node at (-1.3,3.3)  {$ w_2 $};
\node at (0.3,3.3)  {$ \cdots $};
\node at (2.3,3.3)  {$ w_{2\frac{n}{\log n}} $};
\node at (4.3,3.3)  {$ w_{2\frac{n}{\log n}+1} $};
\node at (-2.3,4.3)  {$ x_1 $};
\node at (-1.3,4.3)  {$ x_2 $};
\node at (0.3,4.3)  {$ \cdots $};
\node at (2.3,4.3)  {$ x_{2\frac{n}{\log n}} $};
\node at (4.3,4.3)  {$ x_{2\frac{n}{\log n}+1} $};
%\node at (-0.5,0) {1};
%\node at (4.5,0) {2};
%\node at (2.5,1.2) {3};
%\node at (2,3.3) {4};
%%% edges
\draw[thick] (-2,0) -- (0,1);
\draw[thick] (-1,0) -- (0,1);
\draw[thick] (1,0) -- (0,1);
\draw[thick] (2,0) -- (0,1);

\draw[thick] (-2,3) -- (0,1);
\draw[thick] (-1,3) -- (0,1);
\draw[thick] (0,3) -- (0,1);
\draw[thick] (4,3) -- (0,1);
\draw[thick] (2,3) -- (0,1);

\draw[thick] (-2,3) -- (-2,4);
\draw[thick] (-1,3) -- (-1,4);
\draw[thick] (0,3) -- (0,4);
\draw[thick] (2,3) -- (2,4);
\draw[thick] (4,3) -- (4,4);
\end{tikzpicture}
\end{center}
Coloring interprets the two different sides of the cut.
We can assume without loss of generality that: 
\[
\begin{cases}
cost(w_i,x_i) =3 \ \forall i \in[2\frac{n}{\log n}+1]\\
cost(w_i,u) = 2 \ \forall i \in[2\frac{n}{\log n}+1]\\
\sum_{i\in [n^{0.2}]} cost(v_i,u)\le 1
\end{cases}
\]

Given this graph we can construct the following history sequence:
\[
\mathcal{H}:=\left[\sigma_1,\cdots,\sigma_{h},\quad\text{where $h=\leng(\mathcal{H})$}\right]
\]
\[
\mathcal{H}:=
\underbrace{\boxed{w_1, u ,\boxed{v_{i_{1,1}},v_{i_{1,2}},\cdots}}}_{\text{block $1$}}
\underbrace{\boxed{w_2, u,\boxed{v_{i_{2,1}},v_{i_{2,2}},\cdots}}}_{\text{block $2$}}
\cdots
\underbrace{\boxed{w_{\frac{2n}{\log n}+1}, u ,\boxed{v_{i_{\frac{2n}{\log n}+1,1}},v_{i_{\frac{2n}{\log n}+1,2}},\cdots}}}_{\text{block $\frac{2n}{\log n}+1$}}
\]
To finalize the history sequence $\mathcal{H}$, we will follow the below process:
\begin{itemize}
    \item 
    The first appearance of $v_1$ is chosen randomly between block $1$ and $n^{0.1}$\\
    Every other appearance of $v_1$ has frequency $n^{0.1}$
    
    \item 
    The first appearance of $v_2$ is chosen randomly between block $1$ and $1+n^{0.1}$\\
    Every other appearance of $v_2$ has frequency $n^{0.1}+1$
    
    \item $\vdots$
    \item 
    The first appearance of $v_{n^{0.2}}$ is chosen randomly between block $1$ and $n^{0.2}+n^{0.1}$\\
    Every other appearance of $v_{n^{0.2}}$ has frequency $n^{0.2}+n^{0.1}-1$
%    \todo{Xinzhi: I think every initial block is chosen from $[1,i+n^{0,1}-1]$}
\end{itemize}

For any sequence of moves $L$, a vertex that appears only once in
$L$ is called a singleton; vertices that appear at least twice are called
repeated vertices. Let $\leng(L)$ be the length of L; Let $s_1(L)$ be the
number of singletons in $L$, and let $s_2(L)$ be the number of repeated
vertices in L. Denote by $s(L) = s_1(L) + s_2(L)$ the total number of
distinct vertices that appear in $L$. Finally we will denote $|S|$, the cardinality of 
a set $S$.

\begin{lemma}
For every subsequence $B:=\left[\sigma_{i+1},\cdots,\sigma_{i+|B|}\right]$ of $\mathcal{H}$, it holds:
\[
\frac{S_2(B)}{\leng(B)}\le \Theta(\frac{1}{\log n})
\], i.e $B$ is $\log n$-repeating sequence.
\end{lemma}
\begin{proof}
This argument holds in expectation.%\todo{Xinzhi\&Chenhao: could you give a quick argument for that}

If we denote the number of blocks that are completely contained in $B$ by $b$, then 
\begin{equation*}
\E[\leng(B)] \le (b+2) \sum_{i=n^{0.1}}^{n^{0.1}+n^{0.2}} \frac{1}{i} \approx 0.1b \log n.
\end{equation*}
%
And the expectation of $S_2$ is 
\begin{equation*}
\E[S_2(B)]\ge b-n^{0.1}.
\end{equation*}
%
So
\begin{equation*}
\frac{\E[S_2(B)] }{\E[\leng(B)]}\le \frac{10}{\log n}.
\end{equation*}


We can argue the inequality stated in Lemma holds with high probability using Bernstein's inequality.
\end{proof}

\begin{lemma}
$\mathbb{E}[\leng(\mathcal{H})]=\Theta(n)$.
\end{lemma}
\begin{proof}
$\forall i\in [\frac{2n}{logn}+1]$, the expected length of block $i$ is
\begin{align*}
    \E[\leng(block ~ i)] = \sum_{j=1}^{n^{0.2}}\Pr[v_j \text{ is in block } i] = \sum_{j=1}^{n^{0.2}}\frac{1}{n^{0.1}+j-1} \approx 0.1\log n ~.
\end{align*}
Therefore, $\E [\leng(\mathcal{H})] \approx \sum_{i=1}^{\frac{2n}{logn}+1}0.1\log n = \Theta(n)$ .
\end{proof}
